Metamorphic Relation Prioritization for Effective Regression Testing

Metamorphic testing (MT) is widely used for testing programs that face the oracle problem. It uses a set of metamorphic relations (MRs), which are relations among multiple inputs and their corresponding outputs to determine whether the program under test is faulty. Typically, MRs vary in their ability to detect faults in the program under test, and some MRs tend to detect the same set of faults. In this paper, we propose approaches to prioritize MRs to improve the efficiency and effectiveness of MT for regression testing. We present two MR prioritization approaches: (1) fault-based and (2) coverage-based. To evaluate these MR prioritization approaches, we conduct experiments on three complex open-source software systems. Our results show that the MR prioritization approaches developed by us significantly outperform the current practice of executing the source and follow-up test cases of the MRs in an ad-hoc manner in terms of fault detection effectiveness. Further, fault-based MR prioritization leads to reducing the number of source and follow-up test cases that needs to be executed as well as reducing the average time taken to detect a fault, which would result in saving time and cost during the testing process.

==> LingPipe/biography.tex <==

%\vskip -2\baselineskip plus -1fil
\begin{comment}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1in,clip,keepaspectratio]{madhu_photo.jpg}}]%
{Madhusudan Srinivasan}
 is currently a PhD student in computer science at Montana State University, USA. He received the Masters of Computer Science degree from Texas A{\&}M University, USA and and a Bachelor degree in Computer Science from Anna University, India. His research interests include software testing, metamorphic testing.
\end{IEEEbiography}

%\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1in,clip,keepaspectratio]{hongchuan-pic.jpg}}]%
{HongChuan Wang}
is currently a master's student pursuing a degree in computer science at Montana State University. He is working on techniques to reduce the computational cost of mutation testing, and applications of mutation testing to large-scale software systems.
\end{IEEEbiography}

%\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1in,clip,keepaspectratio]{psaha_pic.jpg}}]%
{Prashanta Saha}
is currently pursuing a PhD degree in Computer Science at Montana State University, USA. He received his Bachelor degree in Computer Science and Engineering from Rajshahi University of Engineering and Technology (RUET), Bangladesh. His research interests focused on automated test suite generation and test suite minimization, and testing scientific software using Metamorphic testing techniques. 
\end{IEEEbiography}

%\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1in,clip,keepaspectratio]{kg010616-kanewala_upulee-2.jpg}}]%
{Upulee Kanewala} is an Assistant Professor at Montana State University, USA. Her research interests include software testing, metamorphic testing and quality assurance of scientific software. Upulee received her Ph.D. in Computer Science from Colorado State University in 2015, a Master of Science from Purdue University in 2010, and a Bachelor of Engineering from University of Peradeniya, Sri Lanka in 2007. She has published multiple peer-reviewed articles and book chapters on MT including the first paper on automatic detection of MRs. Her address is Gianforte School of Computing, 357 Barnard Hall, Montana State University, Bozeman, MT 59717. Her email is upulee.kanewala@montana.edu
\end{IEEEbiography}
\end{comment}


==> MetamorphicTesting.tex <==

\section{Metamorphic Testing}
% the steps for metamorphic testing
The metamorphic testing has been successfully applied to alleviate the test oracle problem~\cite{chen2004case}. The steps for conducting metamorphic testing is as below:

\begin{enumerate}
    \item The central part in performing metamorphic testing is the generation of metamorphic relation. The necessary property is obtained from the specification of the program under test. The property is represented in the form of relation known as \emph{metamorphic relation}. The metamorphic relation involves the relation between multiple inputs and the corresponding expected output.
    \item The \emph{source test case} is generated using traditional test case generation strategies.
    \item A new test case known as a follow-up test case is generated from the source test case based on the defined metamorphic relation.
    \item The test output from the execution of the source and follow-up test case is validated against the metamorphic relation. The violation of metamorphic relation indicates the presence of a fault in the program.
 \end{enumerate}
 % explaining the steps in the form of example. put an example.
 
 Figure~\ref{fig:sortingMT} shows an example of using metamorphic testing to test a sorting program. The sorting program P performs the functionality of sorting the list of positive numeric values in ascending order. The metamorphic relation for the program P is that shuffling the elements in the list should not change the order of the output. As shown in the figure, suppose the source test case is
 \{1, 2, 3, 4\} which is selected using some test case selection strategy. According to metamorphic relation, the follow-up test case can be generated. The follow-up test case \{3, 2, 4, 1\} is constructed by shuffling the elements in the source test case. After the execution of the source and follow-up test case, the output of the test cases can be verified against the metamorphic relation to check whether $O_s$ is equal to $O_f$. If the metamorphic relation is violated, it can be concluded that the program P is faulty.
 \begin{figure}[h]
\centering
\includegraphics[width=80mm,scale=0.5]{sorting_MT.png}
\caption{\label{fig:sortingMT}MT example}
\end{figure}


% previous successful case studies conducted using MT
Since the inception of metamorphic testing, many case studies have shown that metamorphic testing can indeed alleviate the test oracle problem. Zhou et.al~\cite{zhou2018metamorphic} have shown that metamorphic testing can identify faults in real life example such as Google Maps, Amazon, etc using the concept of metamorphic exploration. Donaldson et.al~\cite{donaldson2016metamorphic} showed that metamorphic testing could identify bugs in the compiler for the OpenGL Shading Language. Furthermore, metamorphic testing has detected faults in several programs, including a bioinformatics program~\cite{srinivasan2018quality}. The latest study by Zhou et.al~\cite{zhou2019metamorphic} have shown that MT could identify an unknown fatal error in real life obstacle system of the Baidu Apollo self-driving software. These examples show that metamorphic testing can detect faults in applications across various domains. 

